CuClarabel: GPU Acceleration for a Conic Optimization Solver

We present the GPU implementation of the general-purpose interior-point solver Clarabel for convex optimization problems with conic constraints. We introduce a mixed parallel computing strategy that processes linear constraints first, then handles other conic constraints in parallel. The GPU solver currently supports linear equality and inequality constraints, second-order cones, exponential cones, power cones and positive semidefinite cones of the same dimensionality. We demonstrate that integrating a mixed parallel computing strategy with GPU-based direct linear system solvers enhances the performance of GPU-based conic solvers, surpassing their CPU-based counterparts across a wide range of conic optimization problems. We also show that employing mixed-precision linear system solvers can potentially achieve additional acceleration without compromising solution accuracy.

==> tables/bench_gpu_opf_large_lp_detail_table.tex <==
\scriptsize
\begin{longtable}{||lcccc||cccc||cccc||}
\caption{\detailtablecaption}
\\
 & &  & & & \multicolumn{4}{c||}{\underline{iterations}}& \multicolumn{4}{c||}{\underline{total time (s)}}\\[2ex] 
Problem & vars. & cons. & nnz(A) & nnz(P)  & ClarabelGPU & ClarabelRs & Gurobi & Mosek & ClarabelGPU & ClarabelRs & Gurobi & Mosek\\[1ex]
\hline
\endhead
\sc{case20758\_epigrids} & 182928 & 56275 & 355508 & 1881 &  \winner  18 &  \winner  18 &   29 &   - &   1.63 &   2.69 &  \winner  1.36 &   -\\ 
\sc{case20758\_epigrids\_\_api} & 182928 & 56275 & 355508 & 1881 &  \winner  18 &  \winner  18 &   28 &   - &   1.61 &   2.67 &  \winner  1.27 &   -\\ 
\sc{case24464\_goc} & 210481 & 63871 & 408258 & 348 &  \winner  22 &   - &   32 &   - &   1.92 &   - &  \winner  1.63 &   -\\ 
\sc{case24464\_goc\_\_api} & 210481 & 63871 & 408258 & 348 &  \winner  21 &   - &   32 &   - &    1.9 &   - &  \winner  1.62 &   -\\ 
\sc{case24464\_goc\_\_sad} & 210481 & 63871 & 408258 & 348 &  \winner  24 &   - &   34 &   - &   17.4 &   - &  \winner   1.7 &   -\\ 
\sc{case30000\_goc} & 213698 & 68919 & 399262 & 372 &   38 &   38 &  \winner  35 &   49 &    2.1 &   5.11 &  \winner  1.04 &   6.73\\ 
\sc{case30000\_goc\_\_api} & 213698 & 68919 & 399262 & 372 &  \winner  30 &  \winner  30 &   35 &   46 &   2.02 &   4.65 &  \winner  1.29 &   6.49\\ 
\sc{case30000\_goc\_\_sad} & 213698 & 68919 & 399262 & 372 &  \winner  25 &  \winner  25 &   30 &   67 &   1.88 &   3.31 &  \winner  0.988 &   11.1\\ 
\sc{case78484\_epigrids} & 685984 & 211266 & 1334253 & 0 &  \winner  29 &  \winner  29 &   47 &   - &  \winner  7.69 &   29.3 &   26.9 &   -\\ 
\sc{case78484\_epigrids\_\_api} & 685984 & 211266 & 1334253 & 0 &  \winner  26 &  \winner  26 &   28 &   - &  \winner  7.48 &     27 &   20.2 &   -\\ 
\sc{case78484\_epigrids\_\_sad} & 685984 & 211266 & 1334253 & 0 &  \winner  30 &  \winner  30 &   42 &   - &  \winner  7.89 &   30.4 &   21.4 &   -\\ 
\end{longtable}


==> tables/bench_gpu_opf_large_lp_sgm.tex <==
\begin{tabular}{llcccc}
  \hline
   &  & \textbf{ClarabelGPU} & \textbf{ClarabelRs} & \textbf{Gurobi} & \textbf{Mosek} \\\hline
  Shifted GM & Full Acc. & 1.05 & 6.72 & 1.0 & 33.47 \\
   & Low Acc. & 1.05 & 4.54 & 1.0 & 8.13 \\
  Failure Rate (\%) & Full Acc. & 0.0 & 27.3 & 0.0 & 72.7 \\
   & Low Acc. & 0.0 & 18.2 & 0.0 & 27.3 \\\hline
\end{tabular}

